Pointerformer: Deep Reinforced Multi-Pointer Transformer for the Traveling Salesman Problem

Traveling Salesman Problem (TSP), as a classic routing optimization problem originally arising in the domain of transportation and logistics, has become a critical task in broader domains, such as manufacturing and biology. Recently, Deep Reinforcement Learning (DRL) has been increasingly employed to solve TSP due to its high inference efficiency. Nevertheless, most of existing end-to-end DRL algorithms only perform well on small TSP instances and can hardly generalize to large scale because of the drastically soaring memory consumption and computation time along with the enlarging problem scale. In this paper, we propose a novel end-to-end DRL approach, referred to as Pointerformer, based on multi-pointer Transformer. Particularly, Pointerformer adopts both reversible residual network in the encoder and multi-pointer network in the decoder to effectively contain memory consumption of the encoder-decoder architecture. To further improve the performance of TSP solutions, Pointerformer employs both a feature augmentation method to explore the symmetries of TSP at both training and inference stages as well as an enhanced context embedding approach to include more comprehensive context information in the query. Extensive experiments on a randomly generated benchmark and a public benchmark have shown that, while achieving comparative results on most small-scale TSP instances as SOTA DRL approaches do, Pointerformer can also well generalize to large-scale TSPs.

==> 6Ablation.tex <==
%\subsection{Ablation study}
%In this section, we perform additional ablation studies to assess the key elements of the proposed \name algorithm. 

%In order to show the influence to the performance of \name, 

In this section we present some ablation experiment results that explain some important choices of our approach.

\textbf{Importance of different components of \name}
To assess the influence of some key components to the performance of \name, we carry out an additional ablation study to compare \name and its four variants on instances from \textbf{TSP\_random} with 200 nodes (TSP\_random200). The results are summarized in Table~\ref{tab:ablations}. The first variant only uses the coordinates of each node as inputs without any feature augmentation (denoted by w.o. feature augmentation in the table). The second variant removes the embedding of the current partial route from the context embedding (denoted by w.o. enhanced context embedding). %The third variant applies the REINFORCE algorithm without using the variance-consistent normalization

% \begin{wraptable}{r}{0.5\textwidth}
    % \vspace{-5pt}
\begin{table}[H]
    \centering
    \caption{Ablations of three key elements of \name on TSP\_random200.}
    % \vspace{-2pt}
    % \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|c|c}
        \bottomrule
        Algorithm & Len & Gap\\
        \hline
        \name & 10.793 & 0.68\% \\
        w.o. feature augmentation & 10.813 & 0.87\% \\
        w.o. enhanced context embedding & 11.013 & 2.73\% \\
        %w.o. consistent variance & 10.794 & 0.69\% \\
        w.o. multi-pointer network & 10.797 & 0.72\% \\
        %add enhanced multi-pointers & \textbf{10.783} & \textbf{0.59\%} \\
        \bottomrule
    \end{tabular}
    \label{tab:ablations}
    % }
\end{table}
    %\vspace{-10pt}
% \end{wraptable}

And the third variant does not use the multi-pointer networks, denoted by w.o. multi-pointer network. From Table \ref{tab:ablations}, it is clear that \name achieves the best performance comparing to all the variants, which indicates all components play positive roles to our algorithm. Furthermore, we apply these models directly test the instances from \textbold{TSPLIB} and provide their comparisons in Figure \ref{Fig:ablation}. \name with all components outperforms the three variants, indicating that these components are also important for the generalization of \name.

\begin{figure}[!htb] 
    \centering %图片居中
    \includegraphics[width=0.5\textwidth]{pic/ablation_tsplib.pdf}
    \caption{Ablations of three key elements of \name on TSP\_random200.}
    \l
abel{Fig:ablation} 
\end{figure}

\textbf{How $C$ affects the performance} As we mentioned before, the value of $C$ in Eq.~(\ref{eq:clip}) affects the entropy of distributions over nodes that are to be visited, which consequently has a big impact on the trade-off between exploitation and exploration. As shown in Figure~\ref{Fig.comparison}, once $C$ is too small ($\le 10$ in our experiment on instances from \textbf{TSP\_random} with 100 and 200 nodes), namely, it encourages exploitation too much, then the algorithm will quickly fall into a local optima. However, once $C$ is big enough ($\ge 50$), the difference will be negligible and the algorithm will constantly converge to a better policy than the one for $C=10$.

\begin{figure}[H] 
    \centering %图片居中
    % \includegraphics[width=0.9\textwidth]{pic/clip_value.png}
    \subfloat[TSP\_random100]{\includegraphics[width=0.47\textwidth]{pic/clip_value_tsp100.png}}\quad
	\subfloat[TSP\_random200]{\includegraphics[width=0.47\textwidth]{pic/clip_value_tsp200.png}}\quad
	
    \caption{Comparison of different clipping values. } 
    \label{Fig.comparison} 
\end{figure}







  



% From Table \ref{tab:ablations}, it is clear that \name achieves the best performance comparing to all the variants, which indicates all components play positive roles to our algorithm. Furthermore, the enhanced context embedding has the greatest impact among the four components, followed by the feature augment and multi-pointer network. The enhanced context embedding and the multi-pointer network are used together to predict the probability distribution of the nodes, so they are particularly useful in auto-regressive decoding of nodes. 

%Besides, we found that clipping value $C$ is an interesting parameter in the multi-pointer that can influence the exploration and exploitation of the model. The entropy of output distribution decreases with the increase of clipping value due to the maximum suppression of softmax. 
%The change of clipping value does not affect other parameters of the model, so it is an appropriate factor to control exploration and exploitation like $\epsilon$ in $\epsilon$ -greedy algorithm. 



%The experimental results in Table 4 show that the effect of query improvement is the most obvious, followed by feature enhancement. Consistent variance can get a small improvement. The multi-pointer effect also has a small improvement, but the enhanced multi-pointer effect is more obvious. With the exception of enhanced multi-pointers, these approaches do not substantially increase memory or reduce speed.

%In order to demonstrate the effectiveness of our approach, we performed ablation experiments on feature augment, query enhancement, REINFORCE improvement and multi-pointer respectively. We chose to experiment on TSP200 because of limited resources.

%The AM has high computational complexity and memory complexity due to the transformer architecture with self-attention. For a graph with $N$ nodes, the complexity of the $n_l$ layers encoder with $n_h$ hidden state is $O(N^2\cdot n_h\cdot n_l)$. The running time and memory will increase quadratically with the graph size. For the decoder, Multi-head attention is used to acquire information from the visited nodes in each step. Therefore, the decoder complexity is $O(N^3\cdot n_h)$ for TSP with $N$ nodes. Through memory complexity analysis and experiments, we consider that the AM is difficult to be used in large-scale problems although it performs well in small-scale problems.

%For eAM, we use the reversible residual network in the encoder to reduce memory. The memory complexity of the encoder is $O(N^2\cdot n_h)$ which removes the number of encoder layers. We use the sum of the visited nodes embedding instead of Multi-head attention in the decoder to obtain the information in the graph. The complexity of the decoder is reduced to $O(N^2\cdot n_h)$. We conduct experiments on TSP100 to compare the changes in memory and inference time with same parameters. As can be seen from Figure(\ref{Fig.comparison}), the memory of eAM is about $\frac{1}{3}$ of AM, and the inference time is less. Less memory means we can set a larger batch size to handle more instances at the same time. With the increase of scale, this gap will expand further. Therefore, our model is more suitable for large-scale TSP problems than AM in memory and inference time. 



\iffalse
\begin{table}[!htb]
    \centering
    \caption{Comparison of memory and time consumption between \name and POMO/AM. }
    \begin{tabular}{ccccc}
    \hline
           & \multicolumn{2}{c}{\name} & \multicolumn{2}{c}{POMO(AM)} \\
           & Mem.(Mib)   & Time(s)   & Mem.(Mib)      & Time(s)     \\ \hline
    TSP20  & \textbf{1243} & \textbf{5.82} & 1287 & 36.86\\
    TSP50  & \textbf{1589} & \textbf{11.63} & 2205 & 69.00 \\
    TSP100 & \textbf{3099} & \textbf{51.34}  & 7199 & 130.20\\
    TSP200 & \textbf{13274} & \textbf{324.2} & OOM & - \\ \hline
    \end{tabular}
\end{table}
\fi    

%从表4的实验结果可以看出query改进的效果最为明显，特征增强其次。方差一致可以获得较小的的提升。多指针效果同样有较小的提升，但是强化的多指针提升较为显著。除了强化的多指针，这些方法基本不会增加显存或者降低速度。
%The experimental results in Table 4 show that the effect of query improvement is the most obvious, followed by feature enhancement. Consistent variance can get a small improvement. The multi-pointer effect also has a small improvement, but the enhanced multi-pointer effect is more obvious. With the exception of enhanced multi-pointers, these approaches do not substantially increase memory or reduce speed.


%\subsection{Comparison of convergence rates}
%通过对REINFORCE算法baseline的改进，以及对探索和利用的平衡，我们的算法有着更快的收敛速度。对于TSP问题，每一个实例的解的分布都不相同。在POMO中减去同一实例多个解的均值来降低方差，但是在同一个batch中，不同实例的方差并不相同。这意味着方差越大，实例越重要，这是不合理的。另一方面，在训练过程中advantage的方差越来越小。这导致模型的更新幅度受到影响。因此，我们除以方差以保证分布的一致性。 

%Through the improvement of the REINFORCE algorithm baseline and the balance of exploration and utilization, our algorithm has a faster convergence speed. For TSP problem, the solution distribution of each instance is different. The gap in the length of the optimal solution for different instance may be huge. In POMO, the variance is reduced by subtracting the mean of multiple solutions for the same instance, but in a batch, the variances of different instances is not consistent. This means that the larger the variance, the more important the instance, which is unreasonable. On the other hand, the variance of advantage is getting smaller and smaller during training. This causes the extent of model updates to be affected. Therefore, we divide by the variance to ensure the consistency of the distribution. 

%\subsection{Influence on clipping value}
%在实验中我们发现clipping value对模型有着很大的影响
%In the experiment, we found that clipping value has a great influence on the model. It can control the exploration and exploitation of the model. The entropy of output distribution decreases with the increase of clipping value due to the maximum suppression of softmax. The change of clipping value will not affect other parameters of the model, so it is an appropriate factor to control exploration and exploitation like $\epsilon$ in $\epsilon$ -greedy algorithm. 


